On the De-duplication of LAION-2B

Generative models, such as DALL-E, Midjourney, and Stable Diffusion, have societal implications that extend beyond the field of computer science. These models require large image databases like LAION-2B, which contain two billion images. At this scale, manual inspection is difficult and automated analysis is challenging. In addition, recent studies show that duplicated images pose copyright problems for models trained on LAION2B, which hinders its usability. This paper proposes an algorithmic chain that runs with modest compute, that compresses CLIP features to enable efficient duplicate detection, even for vast image volumes. Our approach demonstrates that roughly 700 million images, or about 30\%, of LAION-2B's images are likely duplicated. Our method also provides the histograms of duplication on this dataset, which we use to reveal more examples of verbatim copies by Stable Diffusion and further justify the approach. The current version of the de-duplicated set will be distributed online.

==> fig_dups.tex <==
% dup_hist_vis
%
\setlength{\myfigsize}{0.15\textwidth}
\begin{figure*}[hbtp]
    \centering  
    \begin{tabular}{c c c c c} % 500 1000 5k 20k >20k
        \includegraphics[width=\myfigsize]{dup_hist_vis/500_0.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/1000_0.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/5000_0.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/20000_0.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/most_0.jpg}
         \\
        \includegraphics[width=\myfigsize]{dup_hist_vis/500_1.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/1000_1.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/5000_1.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/20000_1.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/most_1.jpg}
         \\
        \includegraphics[width=\myfigsize]{dup_hist_vis/500_2.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/1000_2.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/5000_2.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/20000_2.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/most_2.jpg}
         \\
        \includegraphics[width=\myfigsize]{dup_hist_vis/500_3.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/1000_3.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/5000_3.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/20000_3.jpg}&
        \includegraphics[width=\myfigsize]{dup_hist_vis/most_3.jpg}
         \\
         500 & 1000 & 5k & 20k & $>$20k
    \end{tabular}
    \caption{Illustrations of duplicated images.
    In each column, the final row denotes the count of nearly identical duplicates for each sample. The last column may contain anticipated placeholders like the samples in the first and third rows, or typical manufactured items such as ovens. We found that the most duplicated images (100K or more), were typically placeholders indicating a broken image, for which de-duplication is clearly desired. In addition, most images had highly duplicated captions as well. 
    }
    \label{fig:dups_sample}
\end{figure*}

==> fig_multimodal_case.tex <==

\setlength{\myfigsize}{0.4\textwidth}
\begin{figure*}[!htb]
  \centering
    \includegraphics[width=\myfigsize]{results_compression/compression_inzs_pareto_fronts_cpu_vith14_l400m_cpu.png}
    \includegraphics[width=\myfigsize]{results_compression/compression_vs_t2i_pareto_fronts_cpu_vith14_l400m_cpu.png}
  \caption{Investigating the effects of compression on several tasks requiring multi-modality of image features. MSE based compression lose semantics for ImageNet classes at higher compression ratios, w.r.t. to the snip based losses.}
  \label{fig:multimodal failure}
\end{figure*}


==> fig_retrieval.tex <==
\if0
\begin{figure*}[tb]
\includegraphics[width=0.32\textwidth]{results_retrieval/pareto_fronts_cpu_vith14_l400m_cpu.png}
\hspace{0.01\textwidth}
\includegraphics[width=0.32\textwidth]{results_retrieval/pareto_fronts_cpu_vith14_l400m_gpu.png}
\hspace{0.01\textwidth}
\includegraphics[width=0.32\textwidth]{results_retrieval/pareto_fronts_cpu_vitl14_l2b_cpu.png}
\hspace{0.01\textwidth}
\caption{Retrieval Pareto fronts for ViT-H-14 indices on L400M on the CPU (left), GPU (middle) and L2B on CPU (right). All neural based indices outperform autofaiss and an IVFPQ on raw features. On L2B, SNIP and MSE nets perform similarly.}
\label{fig:retrieval bench}
\end{figure*}
\fi

\setlength{\myfigsize}{0.4\textwidth}
\begin{figure*}[tb]
\centering
\includegraphics[width=\myfigsize]{results_retrieval/pareto_fronts_cpu_vith14_l400m_cpu.png}
\includegraphics[width=\myfigsize]{results_retrieval/pareto_fronts_cpu_vith14_l400m_gpu.png}
\includegraphics[width=\myfigsize]{results_retrieval/pareto_fronts_cpu_vitl14_l2b_cpu.png}
\includegraphics[width=\myfigsize]{results_retrieval/pareto_fronts_cpu_vitl14_l2b_gpu.png}
\caption{Retrieval Pareto fronts for ViT-H-14 indices on L400M on the CPU (left), GPU (middle) and L2B on CPU (right). All neural based indices outperform autofaiss and an IVFPQ on raw features. On L2B, SNIP and MSE nets perform similarly.}
\label{fig:retrieval bench}
\end{figure*}

==> fig_sd_overfit.tex <==
\begin{figure*}[hbtp]
\centering
\includegraphics[width=.32\linewidth]{sd_overfit/sylvester_overfit.jpeg}
\hfill
\includegraphics[width=.32\linewidth]{sd_overfit/overfit_2.jpeg}
\hfill
\includegraphics[width=.32\linewidth]{sd_overfit/washer_overfit_sd.jpg} 

\caption{We find several new verbatim copied images by Stable Diffusion (SD), by synthesizing the most copied images on L2B. Left are images duplicated database images and right are synthesized by SD. Top image is highly duplicated (more than 5k times), middle image is moderately duplicated (2000 times) and bottom image is highly duplicated (90k times) yet not verbatim copied.} 
\label{fig:verbatim}
\end{figure*}

==> table_vitb32.tex <==
\begin{table*}[htb]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dimension Reduction & Index Info & Memory (GB) & $R \cap k$%~\eqref{eq:eval r int k} 
& IN Zero-shot Top-1 \\
\hline
Raw ViT-B-32 & - &  239 & 100 &  56.1 \\
\hline
$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 25.4 &  31.4 \\
\hline
$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 35.5 &  34.5 \\
\hline
$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 25.1 &  20.7 \\
\hline
$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 35.4 &  30.4 \\
\hline
OPQ, $d=56$ & AutoFaiss &  2.9 & .05 &  1.0 \\
\hline
OPQ, $d=168$ & AutoFaiss &  5.6 & 21.4 &  23.1 \\
\hline
\end{tabular}
\vspace*{1mm}
\caption{Comparisons of the k-NN accuracy (with k=5) of different networks and losses on ViT-B-32 \cite{radford2021learning} for queries outside of the database vectors, against an exhaustive search. The compressed CLIP features have a dimensionality of $d$, and the number of chunks for product quantization is denoted by $M$.}
\label{tab:vitb32 full analysis}
%\medskip
\end{table*}


==> table_vith14.tex <==
\begin{table*}[tb]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dimension Reduction & Index Info & Memory (GB) & ~\eqref{eq:eval r int k} & IN Zero-shot Top-1 \\
\hline
Raw ViT-H-14 & - &  708 & 100 &  67.1 \\
\hline
$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 29.2 &  40.3 \\
\hline
$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 49.5 &  48.7 \\
\hline
$\mathcal{L}_{\textsc{SNIP}}$, $d=32$ & IVFPQ, M=4 &  2.2 & 36.4 &  39.2 \\
\hline
$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 43.1 &  30.6 \\
\hline
$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 50.1 &  42.3 \\
\hline
$\mathcal{L}_{\textsc{CLIP}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 32.1 &  40.2 \\
\hline
$\mathcal{L}_{\textsc{CLIP}}$, $d=32$ & IVFPQ, M=4 &  2.2 & 28.1 &  39.4 \\
\hline
$\mathcal{L}_{\textsc{CLIP}}$, $d=32$ & IVFPQ, M=8 &  2.9 & 35.5 &  42.2 \\
\hline
$\mathcal{L}_{\textsc{CLIP}}$, $d=8$ & IVFPQ, M=4 &  2.2 & 19.2 &  0.0 \\
\hline
OPQ, $d=56$ & AutoFaiss &  2.2 & 0.1 &  2.7 \\
\hline
OPQ, $d=112$ & AutoFaiss &  2.9 & 1.6 &  8.7 \\
\hline
OPQ, $d=168$ & AutoFaiss &  5.6 & 44.1 &  43.4 \\
\hline
- & IVFPQ, M=4 &  2.4 & 14.6 & 40.4 \\
\hline
- & IVFPQ, M=16 &  5.5 & 44.7 &  46.3 \\
\hline
\end{tabular}
\vspace*{1mm}
\caption{Comparisons of the k-NN accuracy (with k=5) of different networks and losses on ViT-H-14 (OpenClip~\cite{OpenClip}) for queries outside of the database vectors, against an exhaustive search. The compressed CLIP features have a dimensionality of $d$, and the number of chunks for product quantization is denoted by $M$.}
\label{tab:vith14 full analysis}
%\medskip
\end{table*}

\if0
\begin{table*}[tb]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{SOC}  &Dimension Reduction & Index Info & Memory (GB) & ~\ref{eq:eval r int k} & IN Zero-shot Top-1 \\
\hline
&Raw ViT-H-14 & - &  708 & 100 &  67.1 \\
\hline
&$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 29.2 &  40.3 \\
\hline
&$\mathcal{L}_{\textsc{SNIP}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 49.5 &  48.7 \\
\hline
&$\mathcal{L}_{\textsc{SNIP}}$, $d=32$ & IVFPQ, M=4 &  2.2 & 36.4 &  39.2 \\
\hline
&$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 43.1 &  30.6 \\
\hline
&$\mathcal{L}_{\textsc{MSE}}$, $d=128$ & IVFPQ, M=16 &  4.2 & 50.1 &  42.3 \\
\hline
&$\mathcal{L}_{\textsc{CLIP}}$, $d=128$ & IVFPQ, M=4 &  2.2 & 32.1 &  40.2 \\
\hline
&$\mathcal{L}_{\textsc{CLIP}}$, $d=32$ & IVFPQ, M=4 &  2.2 & 28.1 &  39.4 \\
\hline
&$\mathcal{L}_{\textsc{CLIP}}$, $d=32$ & IVFPQ, M=8 &  2.9 & 35.5 &  42.2 \\
\hline
&$\mathcal{L}_{\textsc{CLIP}}$, $d=8$ & IVFPQ, M=4 &  2.2 & 19.2 &  0.0 \\
\hline
&OPQ, $d=56$ & Autofaiss &  2.2 & 0.1 &  2.7 \\
\hline
&OPQ, $d=112$ & Autofaiss &  2.9 & 1.6 &  8.7 \\
\hline
&OPQ, $d=168$ & Autofaiss &  5.6 & 44.1 &  43.4 \\
\hline
&- & IVFPQ, M=4 &  2.4 & 14.6 & 40.4 \\
\hline
&- & IVFPQ, M=16 &  5.5 & 44.7 &  46.3 \\
\hline
\end{tabular}
\caption{NN5 accuracy versus ground truth across networks/losses on ViT-H-14 for queries within the training set.}
\label{tab:vith14 full analysis}
%\medskip
\end{table*}

\fi
